Smoothness Analysis for Probabilistic Programs with Application to Optimised Variational Inference

We present a static analysis for discovering differentiable or more generally smooth parts of a given probabilistic program, and show how the analysis can be used to improve the pathwise gradient estimator, one of the most popular methods for posterior inference and model learning. Our improvement increases the scope of the estimator from differentiable models to non-differentiable ones without requiring manual intervention of the user; the improved estimator automatically identifies differentiable parts of a given probabilistic program using our static analysis, and applies the pathwise gradient estimator to the identified parts while using a more general but less efficient estimator, called score estimator, for the rest of the program. Our analysis has a surprisingly subtle soundness argument, partly due to the misbehaviours of some target smoothness properties when viewed from the perspective of program analysis designers. For instance, some smoothness properties are not preserved by function composition, and this makes it difficult to analyse sequential composition soundly without heavily sacrificing precision. We formulate five assumptions on a target smoothness property, prove the soundness of our analysis under those assumptions, and show that our leading examples satisfy these assumptions. We also show that by using information from our analysis instantiated for differentiability, our improved gradient estimator satisfies an important differentiability requirement and thus computes the correct estimate on average (i.e., returns an unbiased estimate) under a regularity condition. Our experiments with representative probabilistic programs in the Pyro language show that our static analysis is capable of identifying smooth parts of those programs accurately, and making our improved pathwise gradient estimator exploit all the opportunities for high performance in those programs.

==> packages.tex <==
%auto-ignore

\usepackage{cleveref} % for \cref{..}
\usepackage{subcaption} % for \begin{subfigure}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{stmaryrd}
\usepackage{etoolbox} % for \ifstrempty
\usepackage{xspace} % for \xspace
\usepackage{mathbbol} % for \mathbb{abc}
\RequirePackage{paralist}
\usepackage{enumitem}
\usepackage{multirow} % for \multirow
\usepackage{proof} % for \infer
\usepackage{array}
\usepackage{nccmath} % for \medint\int

%%% theorem setting.
\AtEndPreamble{%
  \theoremstyle{acmplain}
  \newtheorem{assumption}{Assumption}
  \theoremstyle{acmdefinition} 
  \newtheorem{remark}[theorem]{Remark}
  \theoremstyle{acmplain}
}

%%% cref setting.
\crefname{assumption}{Assumption}{Assumptions}
\crefname{figure}{Fig{.}}{Figs{.}}%{Figures}
\crefname{table}{Table}{Tables}
\crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{proposition}{Proposition}{Propositions}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{problem}{Problem}{Problems}
\crefname{example}{Example}{Examples}
\crefname{fact}{Fact}{Facts}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{remark}{Remark}{Remarks}
\crefname{condition}{Condition}{Conditions}
\crefname{requirement}{Requirement}{Requirements}
\crefname{enumi}{}{}
%% \crefname{equation}{Eq.}{Eqs.}
\crefname{equation}{Eq{.}}{Eqs{.}}
%% \crefname{section}{{\S}}{{\S}}
\crefformat{section}{\S#2#1#3}
\crefmultiformat{section}{\S#2#1#3}{ and~\S#2#1#3}{, \S#2#1#3}{, and~\S#2#1#3}
\crefformat{appendix}{\S#2#1#3}
\crefmultiformat{appendix}{\S#2#1#3}{ and~\S#2#1#3}{, \S#2#1#3}{, and~\S#2#1#3}
\newcommand{\crefrangeconjunction}{--}


==> pl-pf.tex <==
%auto-ignore

\section{Deferred Results in \S\ref{sec:setup}}

\subsection{Proof of \cref{thm:no-obs-dens}}

\begin{theorem}
  \label{thm:no-obs-dens}
  Let $c$ be an always-terminating command that does not have a double-sampling error and does not have an observe command. Then, for all $\sigma_\theta \in \State[\theta]$,
  \begin{align*}
    \int d\sigma_n\, \pfun{c, \sigma_\theta}{}(\sigma_n)  = 1.
  \end{align*}
\end{theorem}
\begin{proof}
  We will prove the following claim, which implies the claim of the theorem:
  \begin{quote}
  \textsc{Claim-Main:} {\it Let $c$ be a command that does not contain an observe command. Consider a subset $\Sigma_p \subseteq \State[\Var]$ such that for all $\sigma_p \in \Sigma_p$ and $\sigma_n \in \State[\Name]$,
  there exists $\sigma_a \in \State[\AVar]$ satisfying $\sigma_a(\like) = 1$ and $\noerr(c,\sigma_p \oplus \sigma_n \oplus \sigma_a)$. Then,
  \[
  \int d\xi_n\, \getprsub(c)(\sigma_p,\xi_n) = 1
  \quad \text{for every $\sigma_p \in \Sigma_p$}.
  \]
  }
  \end{quote}
  
  This claim, if true, gives the theorem. To see why, consider a command $c$ that always terminates, does not have a double-sampling error, and does not contain an observe command. Define $\Sigma_p \defeq \State[\Var]$. By the termination and double-sampling-error-free properties of $c$, the set $\Sigma_p$ satisfies the condition of the claim. Thus, the claim can be applied to this setup. If we do so, we get the fact that for every $\sigma_p \in \State[\Var]$, 
  \[
  \int d\xi_n\, \getprsub(c)(\sigma_p,\xi_n) = 1.
  \]
  Pick $\sigma_\theta \in \State[\theta]$. Let $\sigma_p \in \State[\PVar \setminus \theta]$ be the state that maps all variables in its domain to $0$. Define $f_* : \State[\Name] \to \State[\AVar]$ be the map that implements the initialisation of auxiliary variables in the definition of $\pfun{c,\sigma_\theta}{}$. Then,
  \begin{align*}
    \int  d\sigma_n\, \pfun{c, \sigma_\theta}{}(\sigma_n) 
    =
    \int  d\sigma_n\, \getpr(c)(\sigma_\theta \oplus \sigma_p,\sigma_n,f_*(\sigma_n))
    =
    \int  d\xi_n\, \getprsub(c)(\sigma_\theta \oplus \sigma_p,\xi_n)
    = 1.  
    \end{align*}
    The first equality is an immediate consequence of the definitions of $\getpr$, $\sigma_p$, and $f_*$, and the second equality follows from \cref{lem:integral-sampled-terms-only} (instantiated with $h = \lambda \sigma'_n.\,1$) and the fact that for all $N \subseteq \Name$,
    \[
    \int d\xi'_n \Big(\ind{\dom(\xi'_n) = \Name \setminus N} \cdot \prod_{\mu \in \dom(\xi'_n)} \cN(\xi'_n(\mu);0,1)\Big) = 1.
    \]
   The last equality comes from the claim.
  
  Let $c$ be a command that does not contain an observe command. We prove our claim by induction on the structure of $c$. Let $\Sigma_p$ be a subset of $\State[\PVar]$ such that for all $\sigma_p \in \Sigma_p$ and $\sigma_n \in \State[\Name]$, there exists $\sigma_a \in \State[\AVar]$ satisfying $\sigma_a(\like) = 1$ and $\noerr(c,\sigma_p \oplus \sigma_n \oplus \sigma_a)$. Pick $\sigma_p \in \Sigma_p$. 
  
  \paragraph{\bf Case $c \equiv \cskip$}
  \paragraph{\bf Case $c \equiv (x:=e)$}
  \paragraph{\bf Case $c \equiv (x:=\csample(n,d,\lambda y.e'))$}
  \paragraph{\bf Case $c \equiv \cobs(d,r)$}
  \paragraph{\bf Case $c \equiv (c';c'')$} This is one of the two difficult cases, with the other case being the one for loops. We start with a proof outline presented as a derivation with equations: 
    \begin{align*}
    &
    \int d\xi_n\, \Big( \getprsub(c';c'')(\sigma_p, \xi_n)\Big)
    \\
    &=
    \int d\xi'_n \Big(
    \getprsub(c')(\sigma_p, \xi'_n) \cdot
    \int d\xi''_n \Big(
    \getprsub(c'')(\getpvarsub(c')(\sigma_p,\xi'_n), \xi''_n)
    \cdot \ind{\dom(\xi'_n) \cap \dom(\xi''_n) = \emptyset}\Big)\Big)
     \\
    &=
    \int d\xi'_n \Big(
    \getprsub(c')(\sigma_p, \xi'_n) 
    \cdot
    \int d\xi''_n \Big(
    \getprsub(c'')(\getpvarsub(c')(\sigma_p,\xi'_n), \xi''_n)\Big)\Big)
    \\
    &=
    \int d\xi'_n  \Big(\getprsub(c')(\sigma_p, \xi'_n)\Big) 
    \\
    & = 1.
  \end{align*}
  The first equality follows directly from \cref{lem:integral-seq-decompose}, if we just set the function $g$ in the lemma to the constant $1$ function. The other equalities are, however, not so easy, and involve non-trivial arguments. Going through the justifications of them form the rest of the proof of this case.
  
  The second equality holds because of the following claim:
  \begin{quote}
  \textsc{Claim-Seq1:} {\it
  For all $\xi'_n,\xi''_n \in \Statesub[\Name]$, if
  \[
  \getprsub(c')(\sigma_p,\xi'_n) \neq 0 \quad\text{and}\quad  
  \getprsub(c'')(\getpvarsub(c')(\sigma_p,\xi'_n), \xi''_n) \neq 0, 
  \]
  then
  $\dom(\xi'_n) \cap \dom(\xi''_n) = \emptyset$.
  }
  \end{quote}
  This claim implies that whenever $\getprsub(c')(\sigma_p,\xi'_n) \neq 0$ and 
  $\getprsub(c'')(\getpvarsub(c')(\sigma_p,\xi'_n), \xi''_n) \neq 0$, the indicator
  function $\ind{\dom(\xi'_n) \cap \dom(\xi''_n) = \emptyset}$ returns $1$, which
  means that we can eliminate the indicator on the LHS of the second equality, as
  we did in the equality. 
  
  Here is the proof of \textsc{Claim-Seq1}. Pick $\xi'_n,\xi''_n \in \Statesub[\Name]$ that satisfy the condition in the claim. Let $\sigma'_p \defeq \getpvarsub(c')(\sigma_p,\xi'_n)$. Since $\getprsub(c')(\sigma_p,\xi'_n) \neq 0$, there exist $\zeta_n \in \Statesub[\Name]$ and $\sigma_a \in \State[\AVar]$ such that
  \[
  \used(c',\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a,\xi'_n).
  \] 
  By \cref{lem:used-sigma-indep} and the assumption on $\sigma_p$, we may assume that
  \[
  \zeta_n(\mu) = \xi''_n(\mu)\ \text{for all}\ \mu \in \dom(\zeta_n) \cap \dom(\xi''_n),
  \quad\text{and}\quad 
  \noerr(c';c'', \sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a).
  \]
  The above $\noerr$ property ensures that $\db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a) \in \State$. In fact, we can characterise
  this output state of $c'$ more accurately:
  \[
  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a) = \sigma'_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a
  \]
  for some $\sigma'_a$ with $\sigma'_a(\like) = 1$; the preservation of $\xi'_n \oplus \zeta_n$ holds by \cref{lem:cnt-increase-and-rv-nochange},
  the property of $\sigma'_a(\like) = 1$ holds by the observe-freeness of $c'$, the equality $\sigma_a(\like) = 1$, and \cref{lem:obs-free-like}),
  and the $\sigma'_p$ in the output state comes from \cref{lem:subfns-well-defined}. 
  The output state satisfies the $\noerr$ predicate:
  \[
  \noerr(c'',\sigma_p' \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a).
  \]
  The reason is that $\db{c''}(\sigma_p' \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a) \in \State$ by
  $\noerr(c';c'', \sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)$, and, also, for all $\mu \in \Name$,
  \begin{align*}
  & \db{c''}(\sigma_p' \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a)(\mu) - (\sigma_p' \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a)(\mu)
  \\
  & \qquad {} = \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - 
   (\sigma_p' \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a)(\mu)
   \\
   & \qquad {} \leq  
   \begin{aligned}[t]
   & \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - 
   (\sigma_p' \oplus \xi'_n \oplus \zeta_n \oplus \sigma'_a)(\mu) 
   \\
   &
   \qquad
   {}
   +
  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu)
  - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu)
  \end{aligned}
  \\
  & \qquad {} =   \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu)
  \\
  & \qquad {} \leq 1.
  \end{align*}
  In the derivation, the first inequality uses \cref{lem:cnt-increase-and-rv-nochange}, and the second
  $\noerr(c';c'', \sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)$.
  Let $\xi'''_n$ be the restriction of $\xi'_n \oplus \zeta_n$ to the following set
  \[
    \{\mu \in \Name \,\mid\, \db{c''}(\sigma'_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a')(\sampled_\mu) -  (\sigma'_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a')(\sampled_\mu) = 1\}
  \]
  and $\zeta'_n$ be $(\xi'_n \oplus \zeta_n)|_{\Name \setminus \dom(\xi'''_n)}$. Then,
  \[
  \used(c'',\sigma'_p \oplus \xi'''_n \oplus \zeta'_n \oplus \sigma'_n, \xi'''_n).
  \]
  Also,
  \[
  \dom(\xi'_n) \cap \dom(\xi'''_n) = \emptyset,\ \text{so that}\ \dom(\xi'''_n) \subseteq \dom(\zeta_n).
  \] 
  If there were $\mu \in \dom(\xi'_n) \cap \dom(\xi'''_n)$, we would have a contradicting conclusion 
  \[
  \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) = 2 
  \]
  as shown in the following derivation:
  \begin{align*}
  & \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  \\
  & \qquad {} = 
  \begin{aligned}[t]
  & \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) -  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu)
  \\ 
  & \qquad {} +  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  \end{aligned}
  \\
  & \qquad {} = 
  \begin{aligned}[t]
  & \db{c''}(\sigma'_p \oplus \xi'''_n \oplus \zeta'_n \oplus \sigma'_a)(\mu) -  (\sigma'_p \oplus \xi'''_n \oplus \zeta'_n \oplus \sigma'_a)(\mu)
  \\ 
  & \qquad {} +  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  \end{aligned}
  \\
  & \qquad = 1 + 1 = 2.
  \end{align*}
  Define $\zeta''_n \in \State[\dom(\zeta'_n)]$ as follows: for all $\mu \in \dom(\zeta'_n)$,
  \[
  \zeta''_n(\mu) 
  \defeq
  \begin{cases}
  \xi''_n(\mu) & \text{if}\ \mu \in \dom(\xi''_n)
  \\
  \zeta'_n(\mu) & \text{otherwise}.
  \end{cases}
  \]
  By \cref{lem:used-sigma-indep}, 
  \[
  \used(c'', \sigma'_p \oplus \xi'''_n \oplus \zeta''_n \oplus \sigma'_a, \xi'''_n).
  \]
  Note that since $\dom(\xi'''_n) \subseteq \dom(\zeta_n)$ and $\zeta_n(\mu) = \xi''_n(\mu)$ for all $\mu \in \dom(\zeta_n) \cap \dom(\xi''_n)$,
  \[
  (\xi'''_n \oplus \zeta''_n)|_{\dom(\xi''_n)} = \xi''_n.
  \]
  Let $\zeta'''_n \defeq (\xi'''_n \oplus \zeta'')|_{\Name \setminus \dom(\xi''_n)}$. Since
  $\used(c'',\sigma'_p \oplus \xi''_n \oplus \sigma_r,\xi''_n)$ for some $\sigma_r$.
  by \cref{lem:used-sigma-indep} again,
  \[
  \used(c'',\sigma'_p \oplus \xi''_n \oplus \zeta'''_n \oplus \sigma'_a, \xi''_n).
  \]
  This, together with $ \used(c'', \sigma'_p \oplus \xi'''_n \oplus \zeta''_n \oplus \sigma'_a, \xi'''_n)$ and the equality $\xi'''_n \oplus \zeta''_n = \xi''_n \oplus \zeta'''_n$,
  implies
  \[
  \xi'''_n = \xi''_n,
  \]
  which gives the desired $\dom(\xi''_n) \cap \dom(\xi'_n) = \emptyset$.
  
  
  Let us go back to the third equality in the outline shown in the beginning of the proof for this sequence case. The equality can be derived by ignoring the case that $\getprsub(c')(\sigma_p,\xi'_n) = 0$, and handling the other case by induction hypothesis on $c''$ with the following set:
  \[
  \Sigma'_p \defeq \{\getpvarsub(c')(\sigma_p,\xi'_n) \,\mid\, \sigma_p \in \Sigma_p \land \exists \sigma_r.\,\used(c',\sigma_p \oplus \xi'_n \oplus \sigma_r, \xi'_n) \}.
  \] 
  To see why we can use induction hypothesis with $\Sigma'_p$, consider $\sigma'_p \in \Sigma'_p$ and $\sigma'_n \in \State[\Name]$. We should show that
  some $\sigma'_a \in \State[\AVar]$ satisfies 
  \[
  \sigma'_a(\like) = 1\quad\text{and}\quad \noerr(c'', \sigma'_p \oplus \sigma'_n \oplus \sigma'_a). 
  \]
  Since $\sigma'_p \in \Sigma'_p$, there exist $\sigma_p \in \Sigma_p$, $\xi'_n \in \Statesub[\Name]$, $\zeta_n \in \State[\Name\setminus \dom(\xi'_n)]$, and $\sigma_a \in \State[\AVar]$ such that 
  \[
  \sigma'_p = \getpvarsub(c')(\sigma_p,\xi'_n)
  \quad\text{and}\quad 
  \used(c',\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a,\xi'_n).
  \]
  By \cref{lem:used-sigma-indep} and the membership $\sigma_p \in \Sigma_p$, we may assume that
  \[
  \zeta_n(\mu) = \sigma'_n(\mu)\ \text{for all}\ \mu \in \dom(\zeta_n),
  \quad\text{and}\quad 
  \noerr(c';c'', (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)).
  \]
  The second conjunct from above implies (via the same argument that we used to handle the second equality in the proof outline)
  \[
  \noerr(c'', \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)).
  \]
  Also, by \cref{lem:subfns-well-defined,lem:cnt-increase-and-rv-nochange,lem:obs-free-like}, 
  \[
  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)
  = \sigma'_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a'
  \]
  for some $\sigma_a'$ with $\sigma_a'(\like) = 1$. 
  Let $\xi''_n$ be the restriction of $\xi'_n \oplus \zeta_n$ to the following set:
  \[
  \{\mu \in \Name \,\mid\, \db{c''}(\sigma'_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a')(\sampled_\mu) -  (\sigma'_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a')(\sampled_\mu) = 1\}
  \]
  and $\zeta'_n$ be $(\xi'_n \oplus \zeta_n)|_{\Name \setminus \dom(\xi''_n)}$. Then,
  \[
  \used(c'',\sigma'_p \oplus \xi''_n \oplus \zeta'_n \oplus \sigma'_a, \xi''_n).
  \]
  We will show that
  \begin{equation}
  \label{eqn:q-integrability:seq-case:1}
  \dom(\xi''_n) \cap \dom(\xi'_n) = \emptyset. 
  \end{equation}
  This implies that $\sigma'_a$ is what we look for, because if we define $\zeta''_n \in \State[\dom(\zeta'_n)]$ by
  \[
  \zeta''_n(\mu) = 
  \begin{cases}
  \sigma'_n(\mu) & \text{if}\ \mu \in \dom(\sigma'_n) \cap \dom(\zeta'_n)
  \\
  \zeta'_n(\mu) & \text{otherwise},
  \end{cases}
  \]
  then $\xi''_n \oplus \zeta''_n = \sigma'_n$ and so, $\used(c'',\sigma'_p \oplus \sigma'_n \oplus \sigma'_a, \xi''_n)$ by \cref{lem:used-sigma-indep},
  which in turn gives
  \[
  \noerr(c'',\sigma_p' \oplus \sigma'_n \oplus \sigma'_a),
  \]
  as desired. For the proof of \cref{eqn:q-integrability:seq-case:1}, suppose that $\dom(\xi''_n) \cap \dom(\xi'_n)$ is not empty, and contains some $\mu$. Then,
  \begin{align*}
  & \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  \\
  & \qquad {} = 
  \begin{aligned}[t]
  & \db{c';c''}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) -  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu)
  \\ 
  & \qquad {} +  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  \end{aligned}
  \\
  & \qquad {} = 
  \begin{aligned}[t]
  & \db{c''}(\sigma'_p \oplus \xi''_n \oplus \zeta'_n \oplus \sigma'_a)(\mu) -  (\sigma'_p \oplus \xi''_n \oplus \zeta'_n \oplus \sigma'_a)(\mu)
  \\ 
  & \qquad {} +  \db{c'}(\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) - (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a)(\mu) 
  \end{aligned}
  \\
  & \qquad = 1 + 1 = 2,
  \end{align*}
  which contradicts to $\noerr(c';c'', (\sigma_p \oplus \xi'_n \oplus \zeta_n \oplus \sigma_a))$. 
  
  It remains to justify the fourth equality in our proof outline for this sequence case. The equality comes from the application of induction hypothesis to $c'$ with $\Sigma_p$. The application is allowed here for the following reason. For all $\sigma_p \in \Sigma_p$ and $\sigma_n \in \State[\Name]$, there exists $\sigma_a \in \State[\AVar]$ such that $\sigma_a(\like) = 1$ and $\noerr(c';c'', \sigma_p \oplus \sigma_n \oplus \sigma_a)$, and this $\sigma_a$ is what we need to justify the application of induction hypothesis because $\noerr(c';c'', \sigma_p \oplus \sigma_n \oplus \sigma_a)$ and \cref{lem:cnt-increase-and-rv-nochange} imply 
  $\noerr(c',\sigma_p \oplus \sigma_n \oplus \sigma_a)$.
  
  \paragraph{\bf Case $c \equiv (\cif\ b\ \{c'\}\ \celse\ c'')$}
  \paragraph{\bf Case $c \equiv (\cwhile\ b\ \{c'\})$} Let $F$ be the operator on $[\State \to \State_\bot]$ defined by
  \[
  F(f)(\sigma) \defeq \text{if}\ (\db{b}\sigma = \strue)\ \text{then}\ f^\dagger(\db{c'}\sigma)\ \text{else}\ \sigma.
  \]
  Define, for every $i \in \N$,
  \[
   f^{(i)} \defeq F^i(\lambda \sigma.\,\bot)
   \quad\text{and}\quad 
   g^{(i)} \defeq F^i(\lambda \sigma.\,\sigma).
   \]
   Note that when $\getprsub$ and $\used$ use their first command argument, they always take the semantics of the argument. We overload $\getprsub$ and $\used$ so that they can take a function in $[\State \to \State_\bot]$ directly. The overloaded $\getprsub$ and $\used$ essentially mean the same as their original counterparts.
   For every $\sigma_p \in \Sigma_p$ and $i \in \N$, let
   \[
   N^{(i)}(\sigma_p) \defeq \{\xi_n \in \Statesub[\Name] \,\mid\,
   \begin{aligned}[t]
   & (\exists \sigma_r.\,\used(f^{(i)}, \sigma_p \oplus \xi_n \oplus \sigma_r, \xi_n))
   \\
   & {} \land
   (i = 0 \vee \neg \exists \sigma_r.\,\used(f^{(i-1)}, \sigma_p \oplus \xi_n \oplus \sigma_r, \xi_n))\}.
   \end{aligned}
   \] 
   
  We point out a few facts on what we have just defined. First, by the definition of $\db{c}$,
  \[
  \db{c} = \bigsqcup_{i \in \N} f^{(i)}.
  \]
  Second, for all $i \geq 0$ and all $\sigma_p \in \Sigma_p$, we have
  \begin{equation}
  \label{eqn:q-integrability:loop-case1}
  \int d\xi_n\, \getprsub(g^{(i)})(\sigma_p,\xi_n) = 1.
  \end{equation}
  This holds because $\Sigma_p$ satisfies the condition of \textsc{Claim-Main} for every $g^{(i)}$, these $g^{(i)}$'s are constructed by sequential composition, if command, $\db{c'}$, and $\cskip$, and by repeating the arguments that we already gave for these language constructs, we can prove \cref{eqn:q-integrability:loop-case1}.
  Third, for every $\sigma_p \in \Sigma_p$,
  \begin{equation}
  \label{eqn:q-integrability:loop-case1b}
  \biguplus_{i \in \N} N^{(i)}(\sigma_p) =
  \{\xi_n \in \Statesub[\Name]\,\mid\, \exists \sigma_r.\,\used(c, \sigma_p \oplus \xi_n \oplus \sigma_r, \xi_n)\}.
  \end{equation}
  Fourth, for all $\sigma_p \in \Sigma_p$ and $i,j \in \N$ with $i \leq j$, and also for all $\xi_n \in N^{(i)}$, 
  \begin{equation}
  \label{eqn:q-integrability:loop-case1c}
  \getprsub(f^{(i)})(\sigma_p, \xi_n) = \getprsub(f^{(j)})(\sigma_p,\xi_n) = \getprsub(c)(\sigma_p,\xi_n) = \getprsub(g^{(j)})(\sigma_p,\xi_n). 
  \end{equation}
  Fifth, for all $\sigma_p \in \Sigma_p$ and $\xi_n \in \Statesub[\Name]$, 
  \begin{equation}
  \label{eqn:q-integrability:loop-case1d}
  \xi_n \not\in \biguplus_{i \in \N} N^{(i)}(\sigma_p)
  \implies (\getprsub(g^{(j)})(\sigma_p,\xi_n) = 0 \ \text{for all}\ j \in \N).
  \end{equation}
   
  Using these facts, we now derive the desired conclusion. By the third, fourth, and fifth facts, we have
  \begin{equation}
  \label{eqn:q-integrability:loop-case2}
  \lim_{i \to \infty} \getprsub(g^{(i)})(\sigma_p,\xi_n) = \getprsub(c)(\sigma_p,\xi_n) 
  \end{equation}
  for all $\sigma_p \in \Sigma_p$ and $\xi_n \in \Statesub[\Name]$. This equality and the second fact (\cref{eqn:q-integrability:loop-case1}) 
  give the desired conclusion as shown below:
  \begin{align*}
  \int d\xi_n\, \getprsub(c)(\sigma_p,\xi_n) 
  = \int d\xi_n\, \Big(\lim_{i \to \infty} \getprsub(c^{(i)})(\sigma_p,\xi_n)\Big)
  = \lim_{i \to \infty} \int d\xi_n\, \getprsub(c^{(i)})(\sigma_p,\xi_n)
  = 1.
  \end{align*}
  The first equality follows from \cref{eqn:q-integrability:loop-case2}, and the third from \cref{eqn:q-integrability:loop-case1}. The second equality is tricky, and we prove it using the Vitali convergence theorem. Let $p_0 : \Statesub[\Name] \to (0,\infty)$ be the function defined by
  \[
  p_0(\xi_n) \defeq \prod_{\mu \in \dom(\xi_n)} \cN(\xi_n(\mu);0,1).
  \]
  Then, $p_0$ defines a finite measure on $\Statesub[\Name]$. Using $p_0$, we spell out one consequence of the Vitali convergence theorem that we use
  to justify the second equality in our derivation from above.
  \begin{quote}
  \textsc{Consequence of Vitali:}
  Let $h,h^{(0)},h^{(1)},\ldots,h^{(i)},\ldots$ be measurable functions of type $\Statesub[\Name] \to [0,\infty)$ such that
  (i) $\int d\xi_n\, p_0(\xi_n) h^{(i)}(\xi_n) < \infty$ for all $i \in \N$, (ii) $\lim_{i \to \infty} h^{(i)}(\xi_n) = h(\xi_n)$ for all $\xi_n \in \Statesub[\Name]$, and (iii) the family $\{h^{(i)}\}_{i \in \N}$ is uniformly integrable, that is,
  \[
  \forall \epsilon > 0.\,\exists B_\epsilon > 0.\,\sup_{i \in \N} \int d\xi_n\, \Big(p_0(\xi_n) \cdot \ind{h^{(i)}(\xi_n) > B_\epsilon} \cdot h^{(i)}(\xi_n)\Big) < \epsilon.
  \] 
  Then,  $\lim_{i \to \infty} \int d\xi_n\, p_0(\xi_n) h^{(i)}(\xi_n) = \int d\xi_n\,p_0(\xi_n) h(\xi_n)$.
   \end{quote}
   Pick $\sigma_p \in \Sigma_p$. We use the above consequence of Vitali with 
   \[
   h(\xi_n) \defeq \getprsub(c)(\sigma_p,\xi_n)/p_0(\xi_n) 
   \quad\text{and}\quad 
   h^{(i)}(\xi_n) \defeq \getprsub(g^{(i)})(\sigma_p,\xi_n)/p_0(\xi_n).
   \]
   Note that the conclusion of the consequence gives the desired $\int d\xi_n\,\getprsub(c)(\sigma_p,\xi_n) = 1$. We now have to show that our $h$ and $h^{(i)}$ satisfy the three conditions of the consequence. Doing so for the first two conditions is easy. For all $i \in \N$, by \cref{eqn:q-integrability:loop-case1},
   \[
   \int d\xi_n\, p_0(\xi_n) h^{(i)}(\xi_n) =  \int d\xi_n\, p_0(\xi_n) h^{(i)}(\xi_n) = \int d\xi_n\, \getprsub(g^{(i)})(\sigma_p,\xi_n) = 1 < \infty.
   \]
   Also, by \cref{eqn:q-integrability:loop-case2}, for all $\xi_n \in \Statesub[\Name]$,
   \[
   \lim_{i \to \infty} h^{(i)}(\xi_n) = \Big(\lim_{i \to \infty} \getprsub(g^{(i)})(\sigma_p,\xi_n)\Big) / p_0(\xi_n) = \getprsub(c)(\sigma_p,\xi_n)/p_0(\xi_n) = h(\xi_n).
   \]
   To show the third uniform-integrability condition, pick $\epsilon > 0$. Let $R^{(i)} \defeq \int d\xi_n\,p_0(\xi_n) h^{(i)}(\xi_n) \ind{\xi_n \in N^{(i)}}$. Then,
   by \cref{eqn:q-integrability:loop-case1,eqn:q-integrability:loop-case1c}, $\{R^{(i)}\}_{i \in \N}$ is an increasing sequence of non-negative reals that is bounded from above by $1$. Thus, it converges, and this convergence implies the existence of some $i_0 \in \N$ with 
   \[
   \int d\xi_n\,p_0(\xi_n) h^{(i_0)}(\xi_n) \ind{\xi_n \not\in N^{(i_0)}} < \epsilon / 2.
   \]
   \hy{I am here.}
\end{proof}

